An Analysis of How COVID-19 Shaped the Realm of Online Gaming and Lesson Delivery

The COVID-19 pandemic has forced schools and universities to adapt to remote learning, and online gaming has emerged as a tool for education. Educational games can make learning fun and engaging, help students develop important skills like problem-solving and collaboration, and reach students who are struggling with traditional learning methods. While there are concerns about the potential drawbacks of online gaming in education, its benefits are clear. As the pandemic continues to disrupt education, online gaming is likely to become an increasingly important tool for teachers and students alike.

==> performanceAssessment.tex <==
\section{Performance Assessment} \label{sec:perf}
After developing our method, we evaluate the performance of through a cross validation. The evaluation results exhibit acceptable accuracy 
